Modified Frame Reconstruction Algorithm for Compressive Sensing

Compressive sensing is a technique to sample signals well below the Nyquist rate using linear measurement operators. In this paper we present an algorithm for signal reconstruction given such a set of measurements. This algorithm generalises and extends previous iterative hard thresholding algorithms and we give sufficient conditions for successful reconstruction of the original data signal. In addition we show that by underestimating the sparsity of the data signal we can increase the success rate of the algorithm. We also present a number of modifications to this algorithm: the incorporation of a least squares step, polynomial acceleration and an adaptive method for choosing the step-length. These modified algorithms converge to the correct solution under similar conditions to the original un-modified algorithm. Empirical evidence show that these modifications dramatically increase both the success rate and the rate of convergence, and can outperform other algorithms previously used for signal reconstruction in compressive sensing.

==> cs.tex <==

\section{Compressive Sensing}
Let $\x\in\R^n$ be a signal and let $\Phi\in\Rmn$ be a measurement matrix.  We call the vector $\y\in\R^m$ the vector of observations if $\y = \Phi \x + \e$ where $\e\in\R^m$ is a vector of noise or errors, possibly equal to $\vec{0}$.  The task is to recover $\x$ given only the observations $\y$ and the matrix $\Phi$.  Clearly if $\e=\vec{0}$, $m=n$ and the columns of $\Phi$ are linearly independent, then $\Phi$ is invertible and $\x$ can be recovered exactly.  However compressive sensing asks (and answers) the question, how well can we do if $m \ll n$?

First, let us define the \emph{Restricted Isometry Property} (RIP) condition of order $s$ for a matrix $\Phi\in\Rmn$ as per \cite{Candes2006a}.  Let $\delta_s\ge 0$ be the smallest value such that
\begin{equation}
	(1-\delta_s) \norm{l2}{\x}^2 \le \norm{l2}{\Phi\x}^2 \le (1+\delta_s) \norm{l2}{\x}^2,
\end{equation}
for all $s$-sparse vectors.  We call $\delta_s$the \emph{restricted isometry constant of order $s$}.  If $\delta_s<1$ we say that $\Phi$ satisfies the RIP of order $s$.  It is easy to see that we have
\begin{equation}
	\lambda_{\min}\left(\Phi^\trans\Phi\right) \le 1-\ds \le 1+\ds \le \lambda_{\max}\left(\Phi^\trans\Phi\right),
\end{equation}
for any $s$.  For a given matrix $\Phi$ the restricted isometry constant $\delta_s$ can be calculated by
\begin{equation}
	\ds = \max_{\Gamma\colon \abs{\Gamma} = s} \left\{ 1-\lambda_{\min}\left(\Phi_\Gamma^\trans\Phi_\Gamma\right),\ \lambda_{\max}\left(\Phi_\Gamma^\trans\Phi_\Gamma\right) - 1\right\}.
\end{equation}
This is proved in Lemma \ref{lem:eig_values_RIP}.

In order to give some sense to the problem of finding a vector $\x$, given the measurements $\y$ so that $\y=\Phi\x$, we make the assumption that $\x$ is sparse.  In particular we say that $\x$ is $s$-sparse if only $s$ components of $\x$ are non-zero.  We can then cast this question as a minimisation problem
\begin{equation}
	\arg \min_{\xh\in\R^n} \norm{l0}{\xh} \text{ subject to } \y=\Phi\xh.
\end{equation}
The following lemma from \cite{Candes2005a} gives conditions under which the minimiser to the $\ell_0$ minimisation problem above is the same as the solution to $\y=\Phi\x$.
\begin{lem}[Lemma 1.2 of \cite{Candes2005a}] \label{lem:existence}
Let $\Phi\in\Rmn$ be a matrix with RIP constant $\delta_{2s}< 1$ and let $\Gamma$ be an index set with $\abs{\Gamma}\le s$.  Let $\x\in\R^n$ be a vector with support $\Gamma$ and set $\y=\Phi\x$.  Then $\x$ is the unique solution to 
\begin{equation}
	\arg\min_{\xh\in\R^n} \norm{l0}{\xh} \qquad \text{subject to} \qquad \y=\Phi\xh,
\end{equation}
and hence $\x$ can be reconstructed exactly from  $\y$.
\end{lem}

Lemma \ref{lem:existence} only proves the existence of a solution but does not say anything about how to find it.  To solve the $\ell_0$ minimisation programme directly is not computationally feasible and the breakthrough with compressive sensing was to show that the linear programme
\begin{equation}
	\arg\min_{\xh} \norm{l1}{\xh} \text{ subject to } \y=\Phi\xh,
\end{equation}
returns, with high probability, the same solution as the $\ell_0$ minimisation problem \cite{Candes2005,Donoho2006}, which in turn, has the same solution to 
\begin{equation}
	\arg\min_{\xh\in\R^n} \norm{l1}{\y-\Phi\xh},
\end{equation}
given $\y=\Phi\x$, where $\x$ is $s$-sparse and  $\Phi$ has RIP constants of order $3s$ and $4s$ such that $\delta_{3s}+3\delta_{4s}<2$, see \cite{Candes2005}.

%The analysis of this problem relies heavily on the nature of the measurement matrix $\Phi$.   We say that the matrix $\Phi$ satisfies the \emph{Restricted Isometry Property} (RIP) condition of 
%As in \cite{Blumensath08} we will use the \emph{Modified RIP}.  Let $\hat{\Phi}\in\Rmn$ be a matrix satisfying the restricted isometry property for $\delta_s$ and let $\Phi = \frac{\hat{\Phi}}{1+\delta_s}$, then
%\begin{equation}
%	(1-\beta_s) \norm{l2}{\x}^2 \le \norm{l2}{\Phi\x}^2 \le \norm{l2}{\x},
%\end{equation}
%for all $s$-sparse $\x$, where
%\begin{equation}
%	\beta_s = 1 - \frac{1-\delta_s}{1+\delta_s} \le 1,
%\end{equation}
%if $\delta_s \le 1$ and we say that $\Phi$ obeys the \emph{modified restricted isometry property} of order $s$ with constant $\beta_s$.


%\subsection{Measurement matrices}
One question is, what matrices $\Phi$ satisfy the RIP of order $s$?  In general, it is not possible to design a matrix $\Phi$ that satisfies the RIP of a particular order.  It has been shown that certain classes of random matrices will obey the RIP with very high probability.  For example, let the columns of $\Phi$ be sampled uniformly at random from the unit sphere, or let each entry $\Phi_{ij}$ be sampled independently from the Gaussian distribution with mean 0 and variance $\frac 1 m$ \cite{Baraniuk2007b}.  Then  $\Phi$ obeys the RIP of order $s$ with probability at least $1-\mathcal{O}(e^{-m})$ provided that $m \ge \mathrm{C} s \log(n/s)$ for some constant $\mathrm{C}$ \cite{Candes2006c}.  As a rule of thumb, for a Gaussian measurement matrix it suffices to take $m\approx 2s\log n$ so that $\ell_1$ minimisation will work \cite{Donoho2006a}.



